Graph Signal Processing: History, Development, Impact, and Outlook

Graph signal processing (GSP) generalizes signal processing (SP) tasks to signals living on non-Euclidean domains whose structure can be captured by a weighted graph. Graphs are versatile, able to model irregular interactions, easy to interpret, and endowed with a corpus of mathematical results, rendering them natural candidates to serve as the basis for a theory of processing signals in more irregular domains. In this article, we provide an overview of the evolution of GSP, from its origins to the challenges ahead. The first half is devoted to reviewing the history of GSP and explaining how it gave rise to an encompassing framework that shares multiple similarities with SP. A key message is that GSP has been critical to develop novel and technically sound tools, theory, and algorithms that, by leveraging analogies with and the insights of digital SP, provide new ways to analyze, process, and learn from graph signals. In the second half, we shift focus to review the impact of GSP on other disciplines. First, we look at the use of GSP in data science problems, including graph learning and graph-based deep learning. Second, we discuss the impact of GSP on applications, including neuroscience and image and video processing. We conclude with a brief discussion of the emerging and future directions of GSP.

==> GraphSignalProcessing_ HistoryandOutlook/packages.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{amsfonts,amsmath}
% \usepackage{algorithm, algpseudocode}%algorithmic
\usepackage{lmodern}
\usepackage[hidelinks]{hyperref}
\usepackage{bookmark}
\usepackage{color}
\usepackage{blindtext}  
\usepackage{fancyhdr}
\usepackage{titlesec}
\usepackage{etoolbox}

% removes page number from dirst page at every chapter
\patchcmd{\chapter}{\thispagestyle{plain}}{\thispagestyle{empty}}{}{}   

\usepackage[figuresright]{rotating}
\usepackage{caption}
% \usepackage[font=small,labelfont=bf]{caption}
\usepackage{subcaption}
% \usepackage[font=small]{subcaption}
\graphicspath{{figs/}}
%\DeclareGraphicsExtensions{.pdf,.eps,.png}

%\usepackage[resetlabels]{multibib}     % multiple bibliographies (incompatible con \bibentry o \fullcite)
% \newcites{own}{Author Bibliography}

% \usepackage[nottoc]{tocbibind}      
%         % incluir bibliografía en toc con páginas correctas. tb puede usarse para la lista de figuras

% %\usepackage[toc,page]{appendix}
%\usepackage{appendix}

\usepackage[table, dvipsnames]{xcolor}
\usepackage{multirow}

\usepackage{calc}
\newcounter{mypage}

% \usepackage{ifthen}         % if then construction
% \newboolean{borradorLimpio} 
% \newboolean{versionISBN}

\usepackage{enumitem}       % para modificar la indentación de itemize

\usepackage{verbatim}
\usepackage{fancyvrb}

% \usepackage{nicefrac}

% \usepackage{array}
% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{setspace}

% \usepackage{xspace,amsmath, amssymb,epsfig,syntonly,color,bm,bbm}
\usepackage{graphicx, epsfig}

% \usepackage{xcolor}

% \usepackage{fourier-orns,MnSymbol}
 
% \newlength{\PRLlen}
% \newcommand*\PRLsep[2]{\settowidth{\PRLlen}{#1}\advance\PRLlen by -\textwidth\divide\PRLlen by -3\noindent\hfill\makebox[\the\PRLlen-2cm]{\resizebox{\the\PRLlen}{1pt}{$\filledtriangleleft$}}\raisebox{#2}{#1}\makebox[\the\PRLlen-2cm]{\resizebox{\the\PRLlen}{1pt}{$\filledtriangleright$}}\hfill\bigskip}


% \usepackage{glossary-mcols}

% \usepackage{marvosym}    %\Smiley \Heart \EUR

\usepackage{indentfirst}        % indent first paragraph
